Multilevel Monte Carlo estimators for derivative-free optimization under uncertainty

Optimization is a key tool for scientific and engineering applications, however, in the presence of models affected by uncertainty, the optimization formulation needs to be extended to consider statistics of the quantity of interest. Optimization under uncertainty (OUU) deals with this endeavor and requires uncertainty quantification analyses at several design locations. The cost of OUU is proportional to the cost of performing a forward uncertainty analysis at each design location visited, which makes the computational burden too high for high-fidelity simulations with significant computational cost. From a high-level standpoint, an OUU workflow typically has two main components: an inner loop strategy for the computation of statistics of the quantity of interest, and an outer loop optimization strategy tasked with finding the optimal design, given a merit function based on the inner loop statistics. In this work, we propose to alleviate the cost of the inner loop uncertainty analysis by leveraging the so-called Multilevel Monte Carlo (MLMC) method. MLMC has the potential of drastically reducing the computational cost by allocating resources over multiple models with varying accuracy and cost. The resource allocation problem in MLMC is formulated by minimizing the computational cost given a target variance for the estimator. We consider MLMC estimators for statistics usually employed in OUU workflows and solve the corresponding allocation problem. For the outer loop, we consider a derivative-free optimization strategy implemented in the SNOWPAC library; our novel strategy is implemented and released in the Dakota software toolkit. We discuss several numerical test cases to showcase the features and performance of our novel approach with respect to the single fidelity counterpart, based on standard Monte Carlo evaluation of statistics.

==> settings.tex <==
\RequirePackage{latexsym}
\RequirePackage{amssymb,amsfonts,amsmath,amsthm}
\RequirePackage[dvips]{graphicx,epsfig}
\RequirePackage[T1]{fontenc}
% \RequirePackage{uarial}
\RequirePackage{palatino}
\RequirePackage{times}
\RequirePackage{fancyhdr}
\RequirePackage{sectsty}
\usepackage[ruled]{algorithm2e}
\usepackage{appendix}
\usepackage{amsbsy}
\usepackage{amsfonts}
\usepackage{amsmath}
\usepackage{amsthm}
\usepackage{amssymb}
% \usepackage{uarial}
\usepackage{array}
\usepackage{bm}
\usepackage{caption}
\usepackage[color]{changebar}
\usepackage{datetime}
\usepackage{epsfig}
\usepackage{enumerate}
\usepackage{enumitem}
\usepackage{fancybox,amssymb}
\usepackage{fancyhdr}
\usepackage{floatflt}
\usepackage[OT1]{fontenc}
\usepackage{graphicx}
\usepackage[dvips]{graphicx}
\usepackage{latexsym}
\usepackage{lastpage}
\usepackage{lineno}
\usepackage{multirow}
\usepackage[sort&compress,numbers]{natbib}
\usepackage[nice]{nicefrac}
\usepackage{overpic}
\usepackage{palatino}
\usepackage{pstricks}
\usepackage{ragged2e}
%\usepackage{setspace}
\usepackage{stfloats}
\usepackage{subcaption,amsmath}
\usepackage{threeparttable}
\usepackage{type1cm}
\usepackage{type1ec}
\usepackage{textcomp}
\usepackage{textfit}
\usepackage{upgreek}
\usepackage{multirow}

%
%\renewcommand\appendix{\par
%  \setcounter{section}{0}%
%  \setcounter{subsection}{0}%
%  \setcounter{equation}{0}
%  \gdef\thefigure{\@Alph\c@section.\arabic{figure}}%
%  \gdef\thetable{\@Alph\c@section.\arabic{table}}%
%  \gdef\thesection{\appendixname~\@Alph\c@section}%
%  \@addtoreset{equation}{section}%
%  \gdef\theequation{\@Alph\c@section.\arabic{equation}}%
%}
\def\appendixname{APPENDIX}

\usepackage[textsize=tiny,textwidth=20mm]{todonotes}
\setlength{\marginparwidth}{2cm}
\usepackage{url}
\usepackage[american]{babel}
%\usepackage{hyperref}
\usepackage{dirtytalk}

\theoremstyle{plain}

\newtheorem{theorem}{Theorem}
%\newtheorem{lemma}[theorem]{Lemma}
\newtheorem{lemma}{Lemma}
\newtheorem{corollary}{Corollary}
%\newtheorem{corollary}[theorem]{Corollary}
\newtheorem{remark}[theorem]{Remark}
% -- definitions & examples
\theoremstyle{definition}
%\newtheorem{defi}{Definition}[section]
%\newtheorem{axio}{Axiom}[section]
% -- remarks & axioms
\theoremstyle{remark}
%\newtheorem{rema}{Remark}[section]
\newtheorem{exam}{Example}[section]
% -- algorithms
%\newtheoremstyle{algostyle}% name
%  {}%      Space above, empty = `usual value'
%  {}%      Space below
%  {}%         Body font
%  {}%         Indent amount (empty = no indent, \parindent = para indent)
%  {\bfseries}% Thm head font
%  {}%        Punctuation after thm head
%  {\newline}% Space after thm head: \newline = linebreak
%  {\thmname{#1}\thmnumber{ #2.}}% Thm head spec
%\theoremstyle{algostyle}
%\newtheorem{algo}{Algorithm}
%\newtheorem{algo}[theorem]{Algorithm}

\usepackage{accents}

\usepackage{expl3}
\usepackage{environ}
\ExplSyntaxOn
\seq_new:N \g_appendices_seq% define a sequence for holding the appendices
\NewEnviron{Appendix}{\seq_gput_right:No \g_appendices_seq \BODY}
\newcommand\AddAppendices{% regurgitate the appendices
  \appendix% turn all subsequent sections into appendices
  \seq_map_inline:Nn \g_appendices_seq{##1}
}
\ExplSyntaxOff

% automatically print the appendices at the end of the document
\usepackage{etoolbox}
\AtEndDocument{\AddAppendices}

%\count0=115
%\usepackage[hang]{footmisc}
%\setlength{\footnotemargin}{0in}
%\frenchspacing

\renewcommand{\alpha}{\upalpha}
\renewcommand{\beta}{\upbeta}
\renewcommand{\sigma}{\upsigma}
\renewcommand{\gamma}{\upgamma}
\renewcommand{\phi}{\upphi}
\renewcommand{\mu}{\upmu}
\renewcommand{\epsilon}{\upepsilon}
\renewcommand{\kappa}{\upkappa}
\renewcommand{\xi}{\upxi}
\renewcommand{\eta}{\upeta}
\renewcommand{\lambda}{\uplambda}
\renewcommand{\tau}{\uptau}
\renewcommand{\rho}{\uprho}
\renewcommand{\delta}{\updelta}
\renewcommand{\theta}{\uptheta}
\renewcommand{\upsilon}{\upupsilon}
\renewcommand{\vartheta}{\upvartheta}
\renewcommand{\nu}{\upnu}
\renewcommand{\omega}{\upomega}
\renewcommand{\zeta}{\upzeta}
\renewcommand{\varepsilon}{\upvarepsilon}
\renewcommand{\varphi}{\upvarphi}
\renewcommand{\psi}{\uppsi}

\newcommand\acknowledgements{\section* {ACKNOWLEDGMENTS}%
}

\newcommand\acknowledgement{\section* {ACKNOWLEDGMENT}%
}

